Hydraulic Parameter Estimation for District Heating Based on Laboratory Experiments

In this paper we consider calibration of hydraulic models for district heating systems based on operational data. We extend previous theoretical work on the topic to handle real-world complications, namely unknown valve characteristics and hysteresis. We generate two datasets in the Smart Water Infrastructure laboratory in Aalborg, Denmark, on which we evaluate the proposed procedure. In the first data set the system is controlled in such a way to excite all operational modes in terms of combinations of valve set-points. Here the best performing model predicted volume flow rates within roughly 5 and 10 \% deviation from the mean volume flow rate for the consumer with the highest and lowest mean volume flow rates respectively. This performance was met in the majority of the operational region. In the second data set, the system was controlled in order to mimic real load curves. The model trained on this data set performed similarly well when evaluated on data in the operational range represented in the training data. However, the model performance deteriorated when evaluated on data which was not represented in the training data.

==> fig/results/c_hist_exciting.tex <==

\newcommand{\hist}[2]{
\begin{subfigure}[t]{.44\textwidth}
    \begin{tikzpicture}
    \begin{axis}[
        width=\textwidth,
        height=.7\textwidth,
        xlabel={$e_#1 \left[ \text{\qunit}\right]$},
        ylabel={$\text{count}$},
        ymax = 300,
        xtick=data,
        ybar interval,
        xtick = {-0.8,-0.6,-0.4,-0.2,0,0.2,0.4,0.6,0.8,1.0},
        xmin = -1.0, xmax = 1.0,
        x tick label style={
            rotate=60,
            anchor=east,
        }
    ]
    \addplot+ [hist={
    bins=30,
    }]
    table [y=e#2, col sep=comma] {data/results/error_test_C_exciting_exciting.csv};
    \end{axis}
    \end{tikzpicture}
\end{subfigure}
}

\hist{1}{0}
\hfill
\hist{2}{1}

\hist{3}{2}
\hfill
\hist{4}{3}



==> fig/results/c_scatter_exciting.tex <==

\begin{subfigure}[t]{.49\textwidth}
    \begin{tikzpicture}
    \begin{axis}[
        width=\textwidth,
        height=.7\textwidth,
        ymin = -1.0, ymax = 1.0,
    ]
    %\addplot[only marks, mark=*, orange] table[y=e0, x=v0, col sep=comma] {data/results/error_train_C_exciting_exciting.csv};
    %\addlegendentry{Training data}
    \addplot[only marks, mark=*, blue] table[y=e0, x=v0, col sep=comma] {data/results/error_test_C_exciting_exciting.csv};
    \end{axis}
    \end{tikzpicture}
\end{subfigure}
\hfill
\begin{subfigure}[t]{.49\textwidth}
    \begin{tikzpicture}
    \begin{axis}[
        width=\textwidth,
        height=.7\textwidth,
        ymin = -1.0, ymax = 1.0,
    ]
    \addplot[only marks, mark=*, blue] table[y=e1, x=v1, col sep=comma] {data/results/error_test_C_exciting_exciting.csv};
    \end{axis}
    \end{tikzpicture}
\end{subfigure}

\begin{subfigure}[t]{.49\textwidth}
    \begin{tikzpicture}
    \begin{axis}[
        width=\textwidth,
        height=.7\textwidth,
        ymin = -1.0, ymax = 1.0,
    ]
    \addplot[only marks, mark=*, blue] table[y=e2, x=v2, col sep=comma] {data/results/error_test_C_exciting_exciting.csv};
    \end{axis}
    \end{tikzpicture}
\end{subfigure}
\hfill
\begin{subfigure}[t]{.49\textwidth}
    \begin{tikzpicture}
    \begin{axis}[
        width=\textwidth,
        height=.7\textwidth,
        ymin = -1.0, ymax = 1.0,
    ]
    \addplot[only marks, mark=*, blue] table[y=e3, x=v3, col sep=comma] {data/results/error_test_C_exciting_exciting.csv};
    \end{axis}
    \end{tikzpicture}
\end{subfigure}


==> fig/results/exciting_scatterplots.tex <==
\newcommand{\scatterplot}[5]{
    \begin{tikzpicture}
    \begin{axis}[
        width=\textwidth,
        height=.9\textwidth,
        xlabel={$ v_#5 \left[ \text{no unit}\right]$ },
        ylabel={$ e_#5 \left[ \text{\qunit}\right]$ },
        ymin = -2.5, ymax = 2.5,
        xmin = 0.0, xmax = 1.0,
        xtick={0,0.25,...,1},
        xticklabels={0, , 0.5, , 1},
        ytick = {-2,-1,...,2},
        yticklabels={-2, , 0, , 2},
        grid = major,
    ]
    \addplot[
    #3,
    only marks, 
    mark=*, 
    mark size=0.5pt,
    opacity=0.2,
    ] table[y=#2, x=#1, col sep=comma] {#4};
    \end{axis}
    \end{tikzpicture}
}

\newcommand{\scatterrow}[6]{
    \begin{subfigure}[t]{0.32\textwidth}
        \scatterplot{#1}{#2}{red}{data/results/error_test_A_exciting_exciting.csv}{#6}
        %\caption{#3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \scatterplot{#1}{#2}{green}{data/results/error_test_B_exciting_exciting.csv}{#6}
        %\caption{#4}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \scatterplot{#1}{#2}{blue}{data/results/error_test_C_exciting_exciting.csv}{#6}
        %\caption{#5}        
    \end{subfigure}
}

\scatterrow{v0}{e0}{}{}{}{1}
\scatterrow{v1}{e1}{}{}{}{2}
\scatterrow{v2}{e2}{}{}{}{3}
\scatterrow{v3}{e3}{}{}{}{4}


==> fig/results/hysteresis_plot.tex <==
\newcommand{\hysteresisplot}[5]{
\begin{subfigure}[t]{0.4\textwidth}
    \begin{tikzpicture}
    \begin{axis}[
        scatter,
        xlabel={$ v_#4 \left[ \text{no unit}\right]$ },
        ylabel={$ e_#4 \left[ \text{\qunit}\right]$ },
        only marks,
        width=\textwidth,
        height=.9\textwidth,
        scatter src=explicit symbolic,
        scatter/classes={
            1={mark=*,red},
            -1={mark=*,blue}
        },
        mark size=1.0pt,
        legend entries={+,-},
        legend columns=1,
        legend pos=north west,
        ymin=-0.75,ymax=0.75,
        xmin=0,xmax=1,
        grid = both,
        legend image post style={mark size=2pt, opacity=1},
    ]
    \addplot[opacity=0.2] table[y=#2, x=#1, meta=#3, col sep=comma] {data/results/error_test_B_exciting_exciting.csv};
    \end{axis}
    \end{tikzpicture}
    %\caption{#5}
\end{subfigure}
}

\hysteresisplot{v0}{e0}{sign0}{1}{}
\hfill
\hysteresisplot{v1}{e1}{sign1}{2}{}

\hysteresisplot{v2}{e2}{sign2}{3}{}
\hfill
\hysteresisplot{v3}{e3}{sign3}{4}{}

==> fig/results/scatter_exciting_vs_realistic.tex <==
\newcommand{\scatterplot}[6]{
    \begin{tikzpicture}
    \begin{axis}[
        xlabel={$ v_#1 \left[ \text{no unit}\right]$ },
        ylabel={$ e_#1 \left[ \text{\qunit}\right]$ },
        width=\textwidth,
        height=.6\textwidth,
        ymin = -1.7, ymax = 1.7,
        xmin = 0.0, xmax = 1.0,
        xtick={0,0.25,...,1},
        xticklabels={0, , 0.5, , 1},
        ytick = {-1.5, -1, ...,1.5},
        yticklabels={,-1 , , 0, , 1, },
        grid = major,
    ]
    \draw[fill=green, fill opacity=0.6] (axis cs:#5,-1.7) rectangle (axis cs:#6,1.7);
    \addplot[
    #3, 
    only marks,
    mark=*,
    mark size=0.5pt,
    opacity=0.1,
    ] table[y=e#2, x=v#2, col sep=comma] {#4};
    \end{axis}
    \end{tikzpicture}
}

\newcommand{\scatterrow}[5]{
    \begin{subfigure}[t]{0.4\textwidth}
        \scatterplot{#1}{#2}{red}{data/results/error_test_C_realistic_realistic.csv}{#3}{#4}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.4\textwidth}
        \scatterplot{#1}{#2}{blue}{data/results/error_test_C_realistic_exciting.csv}{#3}{#4}
    \end{subfigure}
}

\scatterrow{1}{0}{0.53}{0.71}{}
\scatterrow{2}{1}{0.36}{0.62}{}
\scatterrow{3}{2}{0.33}{0.49}{}
\scatterrow{4}{3}{0.38}{0.61}{}

